Transfer learning and subword sampling for asymmetric-resource one-to-many neural translation

There are several approaches for improving neural machine translation for low-resource languages: Monolingual data can be exploited via pretraining or data augmentation; Parallel corpora on related language pairs can be used via parameter sharing or transfer learning in multilingual models; Subword segmentation and regularization techniques can be applied to ensure high coverage of the vocabulary. We review these approaches in the context of an asymmetric-resource one-to-many translation task, in which the pair of target languages are related, with one being a very low-resource and the other a higher-resource language. We test various methods on three artificially restricted translation tasks -- English to Estonian (low-resource) and Finnish (high-resource), English to Slovak and Czech, English to Danish and Swedish -- and one real-world task, Norwegian to North S\'ami and Finnish. The experiments show positive effects especially for scheduled multi-task learning, denoising autoencoder, and subword sampling.

==> figures/autoencoders.tikz.tex <==
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathmorphing,decorations.markings}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{patterns}
\usetikzlibrary{fit}

% OBS: Layers are not compatible with onslide animations
\pgfdeclarelayer{background}
\pgfdeclarelayer{main}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% usage: \tikzstyle{shrink} = [onslide=<6>{text height=5cm}]
%\tikzset{onslide/.code args={<#1>#2}{%
%  \only<#1>{\pgfkeysalso{#2}} % \pgfkeysalso doesn't change the path
%}}
\tikzset{ shorten <>/.style={ shorten >=#1, shorten <=#1 } }

% some colors in hex:
%\definecolor{dblue}{HTML}{000492}

%\tikzstyle{vec} = [very thick, text width=17mm, minimum height=6mm, inner sep=0mm]
%\tikzstyle{vecgrid} = [shorten <>=.4mm]
%\tikzstyle{lstm} = [very thick, rounded corners, draw=green, fill=green!20,
%                    text width=15mm, minimum height=5mm, inner sep=0mm,
%                    text centered, font=\small, text=green]
\tikzstyle{hilight} = [draw=red, inner sep=0mm, very thick, rounded corners]
\tikzstyle{pil} = [draw, very thick, ->]

\tikzstyle{subnet} = [draw, very thick, fill=gray!40, minimum height=8mm]
\tikzstyle{att} = [draw, very thick, fill=gray!40, circle, font=\small, inner sep=0.4mm]
\tikzstyle{inout} = [font=\bf]
\tikzstyle{autoencoder} = [color=dgreen, font=\bf]
\tikzstyle{aelink} = [draw=dgreen, very thick]
\tikzstyle{loss} = [color=dblue, font=\bf]
\tikzstyle{losslink} = [draw=dblue, very thick, dotted]
\tikzstyle{wrap} = [inner sep=0mm]
\tikzstyle{legend} = [font=\footnotesize, text width=21mm, align=left]

\resizebox{\textwidth}{!}{%
\begin{tikzpicture}

\newcommand{\encdec}[4]{
\node[subnet, #4] (enc#1) {#2};
\node[subnet, above=10mm of enc#1] (dec#1) {#3};
\draw[thick] (enc#1.north west) -- (dec#1.south east);
\draw[thick] (enc#1.north east) -- (dec#1.south west);
\coordinate (att#1) at ($(enc#1.north)!.5!(dec#1.south)$);
\node[att, at=(att#1)] (att#1) {A};
}

\encdec{1}{Encoder}{Decoder}{};
\encdec{2}{Encoder}{Decoder}{right=27mm of enc1};
\encdec{3}{Decoder}{Encoder}{right=4mm of enc2};
\encdec{4}{Encoder}{Decoder}{right=27mm of enc3};

\node[subnet, right=10mm of dec4] (reco4) {Reconstructor};
\draw[thick] (dec4.north east) -- (reco4.south west);
\draw[thick] (dec4.south east) -- (reco4.north west);
\coordinate (att4) at ($(dec4.east)!.5!(reco4.west)$);
\node[att, at=(att4)] (att4) {A};

% connections for subfig 1
\node[below=5mm of enc1.south, xshift=-4mm, anchor=east, inout] (src1) {Source};
\node[below=5mm of enc1.south, xshift=2mm, att, anchor=center] (noise1) {C};
\node[right=2mm of noise1, autoencoder] (trgin1) {Target};
\node[above=5mm of dec1.north, xshift=-4mm, anchor=east, inout] (trans1) {Target};
\node[above=5mm of dec1.north, xshift=4mm, anchor=west, autoencoder] (ae1) {Target};
\node[above=2mm of trans1, loss] (labeltrans1) {Target};
\node[above=2mm of ae1, loss] (labelae1) {Target};

\coordinate (in) at ($(enc1.south)+(-2mm,0)$);
\draw[pil] (src1) -| (in);
\coordinate (in) at ($(enc1.south)+(2mm,0)$);
\draw[aelink] (trgin1) -- (noise1);
\draw[pil, aelink] (noise1) -- (in);

\coordinate (out) at ($(dec1.north)+(-2mm,0)$);
\draw[pil] (out) |- (trans1);
\coordinate (out) at ($(dec1.north)+(2mm,0)$);
\draw[pil, aelink] (out) |- (ae1);

\draw[losslink] (trans1) to (labeltrans1);
\draw[losslink] (ae1) to (labelae1);

% connections for subfig 2
\node[below=5mm of enc2.south, xshift=-4mm, anchor=east, inout] (src2) {Source};
\node[above=5mm of dec2.north, xshift=4mm, anchor=west, inout] (trans2) {Target};
\node[below=5mm of enc3.south, xshift=4mm, anchor=west, autoencoder] (ae2) {Source};
\node[above=2mm of trans2, loss] (labeltrans2) {Target};

\coordinate (in) at ($(enc2.south)+(-2mm,0)$);
\draw[pil] (src2) -| (in);

\coordinate (out) at ($(dec2.north)+(-2mm,0)$);
\draw[pil] (out) |- (trans2);
\coordinate (backin) at ($(dec3.north)+(2mm,0)$);
\draw[pil, aelink] (trans2) -| (backin);
\coordinate (out) at ($(enc3.south)+(2mm,0)$);
\draw[pil, aelink] (out) |- (ae2);

\draw[losslink] (trans2) to (labeltrans2);
\draw[losslink] (src2) to (ae2);

% connections for subfig 3
\node[below=5mm of enc4.south, xshift=-4mm, anchor=east, inout] (src4) {Source};
\node[above=3mm of dec4.north, inout] (trans4) {Target};
\coordinate (ae4) at (reco4 |- src4);
\node[at=(ae4), autoencoder] (ae4) {Source};
\node[above=2mm of trans4, loss] (labeltrans4) {Target};

\coordinate (in) at ($(enc4.south)+(-2mm,0)$);
\draw[pil] (src4) -| (in);

\draw[pil] (dec4.north) -- (trans4);
\coordinate (backin) at ($(dec3.north)+(2mm,0)$);
\draw[pil, aelink] (reco4) -- (ae4);

\draw[losslink] (trans4) to (labeltrans4);
\draw[losslink] (src4) to (ae4);

\node[wrap, fit=(src1)(trgin1)] (wrap1) {}; 
\node[wrap, fit=(src2)(ae2)] (wrap2) {}; 
\node[wrap, fit=(src4)(ae4)] (wrap4) {}; 

\node[below=2mm of wrap1, font=\footnotesize] (cite1) {(a) \citet{luong2016neural}, this work};
\node[below=2mm of wrap2, font=\footnotesize] (cite2) {(b) \citet{xia2016dual}, \citet{cheng2016semi-supervised}};
\node[below=2mm of wrap4, font=\footnotesize] (cite4) {(c) \citet{tu2016neural}};

\node[legend, right=18mm of ae4, yshift=3mm] (legendaux) {Aux task};
\node[legend, above=1.5mm of legendaux] (legendmain) {Main task};
\node[legend, above=1.5mm of legendmain] (legendloss) {Loss};
\node[legend, above=1.5mm of legendloss] (legendnoise) {Noise model};
\node[legend, above=1.5mm of legendnoise] (legendatt) {Attention};

\draw[pil, aelink] ($(legendaux.west)-(5mm,0)$) -- ++(4mm,0);
\draw[pil] ($(legendmain.west)-(5mm,0)$) -- ++(4mm,0);
\draw[losslink] ($(legendloss.west)-(5mm,0)$) -- ++(4mm,0);
\node[left=3mm of legendnoise.west, att, anchor=center] () {C};
\node[left=3mm of legendatt.west, att, anchor=center] (legendatticon) {A};

\begin{pgfonlayer}{background}
\node[fill=gray!20, fit=(legendatticon)(legendaux)] () {};
\end{pgfonlayer}


\end{tikzpicture}%
}

